Learning Hybrid Interpretable Models: Theory, Taxonomy, and Methods

A hybrid model involves the cooperation of an interpretable model and a complex black box. At inference, any input of the hybrid model is assigned to either its interpretable or complex component based on a gating mechanism. The advantages of such models over classical ones are two-fold: 1) They grant users precise control over the level of transparency of the system and 2) They can potentially perform better than a standalone black box since redirecting some of the inputs to an interpretable model implicitly acts as regularization. Still, despite their high potential, hybrid models remain under-studied in the interpretability/explainability literature. In this paper, we remedy this fact by presenting a thorough investigation of such models from three perspectives: Theory, Taxonomy, and Methods. First, we explore the theory behind the generalization of hybrid models from the Probably-Approximately-Correct (PAC) perspective. A consequence of our PAC guarantee is the existence of a sweet spot for the optimal transparency of the system. When such a sweet spot is attained, a hybrid model can potentially perform better than a standalone black box. Secondly, we provide a general taxonomy for the different ways of training hybrid models: the Post-Black-Box and Pre-Black-Box paradigms. These approaches differ in the order in which the interpretable and complex components are trained. We show where the state-of-the-art hybrid models Hybrid-Rule-Set and Companion-Rule-List fall in this taxonomy. Thirdly, we implement the two paradigms in a single method: HybridCORELS, which extends the CORELS algorithm to hybrid modeling. By leveraging CORELS, HybridCORELS provides a certificate of optimality of its interpretable component and precise control over transparency. We finally show empirically that HybridCORELS is competitive with existing hybrid models, and performs just as well as a standalone black box (or even better) while being partly transparent.

==> expes_pre_black_box_rf_collab.tex <==
\begin{figure*}[htbp]
    \begin{center}
        
  
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.25_acs_employ_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.50_acs_employ_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.75_acs_employ_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.95_acs_employ_ada_boost_collab.pdf}

   
     \vskip 10 pt
     
   \includegraphics[width=0.75\textwidth]{black_boxes_legend_collab.pdf}
   
    \caption{Training and test performances of the \texttt{RandomForestClassifier} black-boxes learnt using the \prebb{} paradigm on the ACS Employment dataset, for different transparency levels. The plots show both average values and standard deviation.} %, for the three datasets.
    
    \label{fig:results_pre_bb_rf_acs_employ}
    
    \end{center}
\end{figure*}

\begin{figure*}[htbp]
    \begin{center}
        
  
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.25_adult_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.50_adult_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.75_adult_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.95_adult_ada_boost_collab.pdf}

   
     \vskip 10 pt
   
    \caption{Training and test performances of the \texttt{RandomForestClassifier} black-boxes learnt using the \prebb{} paradigm on the UCI Adult Income dataset, for different transparency levels. The plots show both average values and standard deviation.} %, for the three datasets.
    
    \label{fig:results_pre_bb_rf_adult}
    
    \end{center}
\end{figure*}

\begin{figure*}[htbp]
    \begin{center}
        
  
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.25_compas_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.50_compas_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.75_compas_ada_boost_collab.pdf}
         \includegraphics[width=0.49\textwidth]{expes_pre_min_coverage_0.95_compas_ada_boost_collab.pdf}

   
     \vskip 10 pt
     
   \includegraphics[width=0.75\textwidth]{black_boxes_legend_collab.pdf}
   
    \caption{Training and test performances of the \texttt{RandomForestClassifier} black-boxes learnt using the \prebb{} paradigm on the COMPAS dataset, for different transparency levels. The plots show both average values and standard deviation.} %, for the three datasets.
    
    \label{fig:results_pre_bb_rf_compas}
    
    \end{center}
\end{figure*}

==> expes_tradeoffs_valid.tex <==
\begin{figure*}[htbp]
    \begin{center}
        
    %\begin{subfigure}{\textwidth}
    %    \centering
    %    \label{fig:results_tradeoff_acs_employ}
    %     \includegraphics[width=0.49\textwidth]{best_prefixes_dataset_acs_employ_train.pdf}
    %    \includegraphics[width=0.49\textwidth]{best_prefixes_dataset_acs_employ_valid.pdf}
    %    \caption{ACS Employment dataset}
    %\end{subfigure}
    
     %\vskip 10 pt
     
    \begin{subfigure}{\textwidth}
        \centering
        \label{fig:results_tradeoffs_adult_valid}
         \includegraphics[width=0.49\textwidth]
         {acc_cov_valid_adult_random_forest.pdf}
        \includegraphics[width=0.49\textwidth]
         {acc_cov_valid_adult_gradient_boost.pdf}
        \caption{UCI Adult Income dataset}
    \end{subfigure}
    
    \vskip 10 pt
    
     \begin{subfigure}{\textwidth}
        \centering
        \label{fig:results_tradoffs_compas_valid}
         \includegraphics[width=0.49\textwidth]
         {acc_cov_valid_compas_random_forest.pdf}
        \includegraphics[width=0.49\textwidth]
         {acc_cov_valid_compas_gradient_boost.pdf}
        \caption{COMPAS dataset}
    \end{subfigure}
    
     \vskip 10 pt
   
     
   \includegraphics[width=0.6\textwidth]{acc_cov_test_legend.pdf}
   
    \caption{Validation set accuracy-coverage trade-offs for various hybrid models and datasets. The Pareto front for each method is represented as a line. (Right) Random Forests, (Left) Gradient Boosted Trees.}
    \label{fig:results_tradeoff_valid}
    
    \end{center}
\end{figure*}
